Bordered Floer homology and contact structures

We introduce a contact invariant in the bordered sutured Heegaard Floer homology of a three-manifold with boundary. The input for the invariant is a contact manifold $(M, \xi, \mathcal{F})$ whose convex boundary is equipped with a signed singular foliation $\mathcal{F}$ closely related to the characteristic foliation. Such a manifold admits a family of foliated open book decompositions classified by a Giroux Correspondence, as described in earlier work of Licata and V\'ertesi. We use a special class of foliated open books to construct admissible bordered sutured Heegaard diagrams and identify well-defined classes $c_D$ and $c_A$ in the corresponding bordered sutured modules. Foliated open books exhibit user-friendly gluing behavior, and we show that the pairing on invariants induced by gluing compatible foliated open books recovers the Heegaard Floer contact invariant for closed contact manifolds. We also consider a natural map associated to forgetting the foliation $\mathcal{F}$ in favor of the dividing set, and show that it maps the bordered sutured invariant to the contact invariant of a sutured manifold defined by Honda-Kazez-Mati\'{c}.

==> construction/old/constructionNEW.tex <==
% !TEX root = ../bordered-contact-main.tex


\section{Construction of the contact invariant}
\label{sec:construction}

\subsection{Bordered manifold associated to a triple}\label{ssec:suturedbordered} 



Let $\mathcal{F}=(\widetilde{\pi}, H=H_+\cup H_-,E)$ be a signed foliation on $\partial M$, and recall that  $(M,\xi,\mathcal{F})$ denotes a contact manifold compatible with the boundary foliation in the sense of  Definition~\ref{def:mxif}. Set $\bsGamma:=\widetilde{\pi}^{-1}(0)$, so that $\bsGamma$ is a disjoint union of oriented leaves $I$ connecting positive elliptic  points $e_+(I)$ to negative elliptic points $e_-(I)$. 
For each component $I$ of $\bsGamma$, define $R_+(I)=\pit^{-1}[0,\epsilon]$ and $R_-(I)=\pit^{-1}[-\epsilon,0]$, where $\epsilon$ is chosen small enough that the interval contains no critical points of $\pit$.  Write  $R_+(\bsGamma)= \bigcup_{I\subset \bsGamma} R_{+}(I)$ and similarly, $R_-(\bsGamma)= \bigcup_{I\subset \bsGamma} R_{-}(I)$.  Set $F=\bdy M\setminus (R_+(\bsGamma)\cup R_-(\bsGamma))$. 





Next, we use the foliation to define a natural parametrization of $F$ via an arc diagram $\zz=(Z,a,m)$. For each positive (negative) hyperbolic point $h_i$, denote the pair of (un)stable separatrices of $\fol$ connecting $h_i$ to the elliptic points by $\delta_i$. Let $Z(I)$ be a pushoff of $\pit^{-1}(-\epsilon)$ 
into $F$ satisfying the following: 
\begin{itemize}
\item $\bdy Z(I)=\left(-e_-(I)\right)\cup e_+(I)$
\item if $\delta_i$ has an endpoint at $e_\pm(I)$, then $Z(I)$ intersects $\delta_i$ in a unique point; otherwise,  $\delta_i$ and $ Z(I)$ are disjoint.
\end{itemize}
Let $Z=\amalg_{I\subset \bsGamma} Z(I)$.  Define $a$ to be the set of all intersection points of $Z$ with the union of the 
$\delta_i$ and let $m$ be the pairing induced on the points in $a$ by $\delta_i$. See Figure~\ref{fig:torus-bs-NEW}. It is easy to check that $\zz=(Z,a,m)$ parametrizes $F$ as a \emph{$\beta$-type arc diagram} as defined in \cite[Definition 3.2]{bs-JG}; i.e., $F$ can be  identified with $F(\mathcal{Z})$. 


\begin{figure}[h]
\begin{center}
\labellist
  	\pinlabel $\textcolor{blue}{\delta_1}$ at 65 55
  	\pinlabel $\textcolor{blue}{\delta_1}$ at 158 100
	\pinlabel $\textcolor{blue}{\delta_2}$ at 158 30
	\pinlabel $\textcolor{blue}{\delta_3}$ at 227 30
	\pinlabel $\textcolor{blue}{\delta_4}$ at 227 100
	\pinlabel $\textcolor{OliveGreen}{e_-}$ at 116 77
	\pinlabel $\textcolor{OliveGreen}{e_+}$ at 116 145
	\pinlabel $\textcolor{OliveGreen}{e_-}$ at 32 90
	\pinlabel $\textcolor{OliveGreen}{e_+}$ at 32 140
	\pinlabel $\textcolor{OliveGreen}{\bsGamma}$ at 116 109
	\pinlabel $Z$ at 211 109
\endlabellist
\includegraphics[scale=1.4]{construction/torus-bs-NEW}
\caption{In this picture, $R_+(\bsGamma)$ and $R_-(\bsGamma)$ are colored with light blue and light red, respectively. Thus $F$ is the union of dark red and white regions. Furthermore, dark red may be identified with $Z\times [0,1/2]$ under the identification of $F$ with $F(\zz)$.}
\label{fig:torus-bs-NEW}
\end{center}
\end{figure} 


\begin{definition}\label{def:fc-bs}
The triple $(M,\bsGamma,\zz)$ described above is the \emph{bordered sutured manifold associated to the foliated contact three-manifold $(M,\xi,\mathcal{F})$}.
\end{definition}


\subsection{Adapted bordered Heegaard diagram}\label{ssec:bordereddiagram}



Let $(\{S_i\}_{i=0}^{2k},h, \{\gamma_i^\pm\})$ be an abstract sorted foliated open book compatible with the foliated contact three-manifold $(M,\xi,\mathcal{F})$.
In what follows, we will describe a generator in a bordered sutured Heegaard diagram $\HH = (\Sigma, \betas,\alphas, \zz)$ constructed from the data of  $(\{S_i\},h, \{\gamma_i^\pm\})$. Let $g_i$ be the genus of $S_i$ and let $n_i$ be the number of boundary components of $S_i$. Recall that  the boundary of the cornered surface $S_i$ is $B\cup A_i$, where $B$ is a union of circles and arcs, and $A_i$ is a union of intervals only. 
 
We let $\Sigma=S_{0}\cup_{B}-S_{0}$.  In order to distinguish the two copies, we will write 
\[\Sigma=S_{\epsilon}\cup_{B}-S_{0},\] 
but we emphasize that $S_\epsilon$ can be identified with $S_0$. The surface $\Sigma$ has genus $2g_0+n_0-1$ and $|A_0|$ boundary components.  For $i\in H_+$, let $\gamma_i^+$ be the $S_{\epsilon}$ copy of the associated sorting arc.  The endpoints of $\gamma_i^+$ lie  near the $E_+$ end of intervals of $A_\epsilon$. Isotope the arcs $\{\gamma_i^+\}$ (simultaneously, to preserve disjointness) near the endpoints along $-\bdy\Sigma$ until they all lie in $I_+\subset A_0$;  the isotopy stops after crossing $E_+$ and before encountering $\cup_{j\in H_-}h(\gamma_j^-)\subset S_0$. Call the resulting arcs $\beta_i^a$. 

For $i\in H_-$, consider the $S_{2k}$ copies of the cutting arcs $\gamma_i^-$, and let $\beta_i^a = -h(\gamma_i^-)$ on $S_0$. 
Write $\betas^a = \{\beta_1^a, \ldots, \beta_{2k}^a\}$.   For convenience, instead of $\beta_i^a$ we will sometimes write $\beta_i^{\pm}$ if $i\in H_{\pm}$.

For $i\in H_{+}$, let $b_i^+ = \beta_i^a\cap S_{\epsilon}$. That is, $b_i^+$ is the arc $\beta_i^a$ with the two end segments that lie on $-S_0$ removed, so that $\partial b_i^+$ lies on $B$.
We claim that after cutting $S_{\epsilon}$ along the arcs $b_i^+$, each connected component contains at least one interval of $A_{\epsilon}$.   

\begin{lemma}\label{lem:cut-gamma}
Each component of  $S_{\epsilon}\setminus \cup_{i\in H_+}b_i^+$ contains an interval component of $A_{\epsilon}$, and hence at least one point in $E_+$, and, equivalently, at least one point in $E_-$. 
\end{lemma}
\begin{proof}
Recall that moving along any given interval of $A_{\epsilon}$, we encounter curves $\gamma_i^+$ indexed in decreasing order. Thus, after the isotopy, moving along any given interval of $B$, we encounter curves $b_i^+$ indexed in decreasing order as well.  Now, suppose there is a component  $C$ of $S_{\epsilon}\setminus \cup_{i\in H_+}b_i^+$ that does not intersect $A_{\epsilon}$. Then the boundary of  $C$ consists of possibly some complete binding circles and at least one circle that alternates between intervals of $B$ and entire arcs $b_i^+$. Since $C$ is a subsurface of $S_{\epsilon}$, the orientation on $B$ agrees with the orientation on $\bdy C$. When traversing this circle of $\bdy C$, it follows  that each interval of $B$ starts at an intersection point with some $b_i^+$ and ends at an intersection point with some $b_j^+$ where $j<i$, thus inducing a circular $<$ ordering on integral indices, which is a contradiction.
\end{proof}

 Let ${\boldsymbol b} = \{b_1, \ldots, b_{2g_0+n_0+|A_0|-k-2}\}$ be a set of cutting arcs for $P_{\epsilon}\subset S_{\epsilon}$ disjoint from $\betas^a$ and with endpoints on $B$, so that each connected component of $S_{\epsilon}\setminus ({\boldsymbol b}\cup \betas^a) = S_{\epsilon}\setminus ({\boldsymbol b}\cup \{b_i^+\}_{i\in H_+})$ is a disk with exactly one interval of $A_{\epsilon}$ on its boundary.
 Note that Lemma~\ref{lem:cut-gamma} guarantees this can be achieved.  In other words, ${\boldsymbol b}$ is a basis for $H_1(P_\varepsilon, B)$. Recalling the identification  $S_\epsilon=S_0$, we may push $b_i\subset S_0$ through $M$ to lie on $S_0$ again and define
   \[\beta_i=b_i\cup -h\circ \iota(b_i)\subset S_{\epsilon}\cup_{B}-S_{0},\]
   where $\iota$ is the identification of $P_0$ with $P_{2k}$ from  Section \ref{sssec:suff}. 
Write $\betas^c=\{\beta_1, \dots, \beta_{2g_0+n_0+|A_0|-k-2}\}$.
  
  Note that by modifying the isotopy that transforms $\{\gamma_i^+\}$ into $\{\beta_i^+\}$, possibly forcing it to happen in a smaller neighborhood of $E_+$, we may assume that all curves in $\betas^a \cup \betas^c$ are pairwise disjoint.

 
 For each cutting arc $b_i\in \boldsymbol b$ on $S_\epsilon$, let $a_i$ be an isotopic curve formed by pushing the endpoints negatively along the boundary so that $a_i$ and $b_i$ intersect once transversely. Similarly, for each arc $b_j^+$, let $\tilde a_j$ be an isotopic curve formed by pushing the endpoints negatively along the boundary so that $\tilde a_j$ and $b_j^+$ intersect once transversely.  We ``double" each of these arcs to form the $\alpha$-circles which define the handlebody $S_0\times [0,\epsilon]$. Namely, define  
  \begin{align*}
 \alpha_i &= a_i\cup -a_i \subset S_{\epsilon}\cup_{B}-S_{0}\\
 \widetilde{\alpha}_j &= \tilde a_j\cup -\tilde a_j \subset S_{\epsilon}\cup_{B}-S_{0},
 \end{align*}

   and write $\alphas^c = \{\widetilde\alpha_i\}_{i\in H_+}\cup \{\alpha_1, \dots, \alpha_{2g_0+n_0+|A_0|-k-2}\}$.
Let $\bsGamma= \bigcup_{I\subset A_{\epsilon}}I\setminus(I_+\cup I_-)$. 

We say that a bordered sutured Heegaard diagram constructed as above is \emph{adapted} to the sorted abstract foliated open book $(\{S_i\},h, \{\gamma_i^\pm\})$. 

Let $\HH = (\Sigma, {\alphas}, {\betas},\zz)$ be a bordered sutured Heegaard diagram adapted to $(\{S_i\},h, \{\gamma_i^\pm\})$.
 Using the  notation introduced above, 
define the set 
\[\xxx = \{x_1, \ldots, x_{2g_0+n_0+|A_0|-k-2}\} \cup \{x_i^+ \mid i\in H_+\}\]
as the unique intersection points 
\begin{align*}
x_i &=  a_i\cap b_i \in S_{\epsilon}\subset \Sigma\\
x_i^+ &= \tilde a_i\cap b_i^+\in S_{\epsilon} \quad \textrm{ if } i\in H_+.
\end{align*}


\begin{example}\label{ex:HeegaardDiagram}
We show the step-by-step construction of the bordered sutured Heegaard diagram adapted to the sorted foliated open book from Example~\ref{ex:sorted}. {To simplify notation, we write $S_i$ and $h$ instead of the $S_i'$ and $h'$ labels used in Example~\ref{ex:sorted}.}

	
	In Figure \ref{fig:HD1_betaplus}, we see the sorting arcs $\gamma_i^+$ and their images $\beta_i^+$ after the isotopy taking their endpoints to $I_+\subset A_0$. The arcs $b_i^+$ are the intersections $\beta_i^+ \cap S_\epsilon$.
	
\begin{figure}[h]
\begin{center}
\includegraphics[scale=0.6]{construction/HD1_betaplusJL}
\caption{The sorting arcs $\gamma_i^+$ (on the left) and their images $\beta_i^+$ (on the right) after the isotopy taking their endpoints to the highlighted subintervals $I_+\subset A_0$. The parts of $\beta_i^+$ lying on $S_\epsilon$ are $b_i^+$.}\label{fig:HD1_betaplus}
\end{center}
\end{figure}
	
	Figure \ref{fig:HD2_betaminus} shows the sorting arcs $\gamma_{i}^-$ on $S_0$ and, after mirroring, their images $\beta_i^- = -h(\gamma_{i}^-)$ on $-S_0$; recall that in this example $h$ is the identity. Recall that $\betas^a = \{\beta_i^{+} \mid i\in H_+\}\cup \{\beta_i^{-} \mid i\in H_-\}$.	
	
	\begin{figure}[h]
		\begin{center}
			\includegraphics[scale=0.61]{construction/HD2_betaminusL}
			\caption{The sorting arcs $\gamma_i^-$ and their images $\beta_i^- = -h(\gamma_{i}^-)$ on $-S_0$.}\label{fig:HD2_betaminus}
		\end{center}
	\end{figure}

	Observe that in this example we do not need any cutting arcs $\boldsymbol b$, because $S_\epsilon\setminus \{b_i^+\}_{i=1,3}$ consists of two disks, each with exactly one interval of $A_\epsilon$ on its boundary, see Figure \ref{fig:HD3_R}. Therefore, $\betas^c$ is empty, and we have no $a_i$ arcs, either.	
	\begin{figure}[h]
		\begin{center}
			\includegraphics[scale=0.61]{construction/HD3_RL}
			\caption{Cutting $S_{\epsilon}$ along $b_i^+$ yields two disks, each with exactly one interval of $A_\epsilon$ on its boundary. Therefore, we do not need any more cutting arcs.}\label{fig:HD3_R}
		\end{center}
	\end{figure}

We next define $\tilde a_i$ by pushing the endpoints of  $b_i^+$ negatively along the boundary so that $\tilde a_i$ and $b_i^+$ intersect once transversely. Figure \ref{fig:HD4_alpha} shows the arcs $\tilde a_i$ on $S_\epsilon$ and their mirror images on $-S_0$. Glued together, they form $\widetilde{\alpha}_i$.  Since this example has no $\alpha_i$ curves, we have $\alphas^c= \{\widetilde\alpha_i\}_{i\in H_+}$.
	
	\begin{figure}[h]
		\begin{center}
			\includegraphics[scale=0.61]{construction/HD4_alphaL}
			\caption{The $\widetilde{\alpha}_i$ curves obtained from the $b_i^+$ arcs.}\label{fig:HD4_alpha}
		\end{center}
	\end{figure}

Finally, Figure \ref{fig:HD5_diagram} illustrates the bordered sutured Heegaard diagram adapted to the sorted  foliated open book of Example \ref{ex:sorted}. In this example, the set of intersection points $\xxx$ consists only of $x_i^+ = \tilde a_i\cap b_i^+\in S_{\epsilon}$ for  $i\in H_+$.

\begin{figure}[h]
	\begin{center}
		\includegraphics[scale=0.61]{construction/HD5_diagramL}
		\caption{The bordered sutured Heegaard diagram adapted to the sorted  foliated open book of Example \ref{ex:sorted}. The intersection points $x_i^+ = \tilde a_i\cap b_i^+\in S_{\epsilon}$ for $i\in H_+$ are marked as black dots.}\label{fig:HD5_diagram}
	\end{center}
\end{figure}
\end{example}

We will use $\xxx$ to define two contact invariants in bordered sutured Floer homology. In order to do that, we first show that $\HH$ is an admissible diagram for the bordered sutured manifold associated to $(M,\xi,\mathcal{F})$. 

\begin{proposition}\label{prop:hd-fc}
Let $(\{S_i\},h, \{\gamma_i^\pm\})$ be a  sorted abstract foliated open book supporting a foliated contact three-manifold $(M,\xi,\mathcal{F})$. 
Suppose $\HH = (\Sigma, \alphas,\betas,\zz)$ is a  bordered sutured Heegaard diagram adapted to $(\{S_i\},h, \{\gamma_i^\pm\})$. Then $\HH$ gives an admissible bordered Heegaard diagram for  the bordered sutured manifold $(M,\bsGamma,\zz)$ associated to $(M,\xi,\mathcal{F})$.
\end{proposition}
\begin{proof} Recall we chose $\bsGamma$ to be the union of arcs $\bigcup_{I\subset A_{\epsilon}}I\setminus(I_+\cup I_-)$. If we instead make the choice $\bsGamma = A_{\epsilon}$, which is equivalent to the original choice up to a small isotopy, then it is immediate from the construction that the Heegaard diagram describes $(M,\bsGamma,\zz)$. \footnote{The reason behind our seemingly unnatural choice is that it allows for a simpler discussion of gluing in Section~\ref{sec:gluing}.} As for admissibility, we notice that just as in the closed or sutured cases, admissibility is automatic:  every periodic domain with an $\alpha$-circle on its boundary crosses the only intersection of that circle with $\betas$ curves or circles on $S_{\epsilon}$, at which point the sign of the connected component of $\Sigma\setminus (\alphas\cup\betas)$ must change.
\end{proof}


If $\HH$ is a bordered  sutured Heegaard diagram adapted to  a sorted abstract foliated open book $(\{S_i\},h, \{\gamma_i^\pm\})$ and  $(\{S_i\},h, \{\gamma_i^\pm\})$ is compatible with the foliated contact three-manifold $(M,\xi,\mathcal{F})$, we say that $\HH$ is \emph{adapted} to $(M,\xi,\mathcal{F})$.



By Proposition~\ref{prop:hd-fc} and \cite[Section 3.4]{bs-JG}, the diagram ${\overline{\HD}=(\Sigma, \betas,\alphas,\overline{\zz})}$ obtained by exchanging the roles of the two sets of curves and formally replacing the arc diagram $\zz$ of $\beta$-type (which is to say, parametrized by arcs which are part of the second set of curves)  with the identical arc diagram $\overline{\zz}$ of $\alpha$-type (parametrized by arcs which are part of the first set of curves) is a bordered sutured diagram for $(-M,\bsGamma,\overline{\zz})$. Write $\overline{\zz}=(Z, a, m)$. We have the following proposition:

 
\begin{proposition}\label{prop:xd-def}
The above $\xxx$ gives a well defined generator
\[
\xxx_D := \xxx\in \bsdhat(\overline{\HH})
\]
with  $I_D(\xxx) = I(H_-)$ and $\delta^1(\xxx_D) = 0$, 
and a well defined generator
\[
\xxx_A  := \xxx\in \bsahat(\overline{\HH})
\]
with $I_A(\xxx_A) = I(H_+)$ and $m_{i+1}(\xxx_A, a(\brho_1), \ldots, a(\brho_i))=0$ for all $i\geq 0$ and all sets of Reeb chords $\brho_j$ in $(Z, a)$.
\end{proposition}
\begin{proof}
Since each of the intersections in the definition of $\xxx$ is unique,  the two generators are well defined. The idempotents are as stated, since the $\beta$-arcs occupied by $\xxx$ are indexed by $H_+$, whereas the unoccupied $\beta$-arcs are indexed by $H_-$. Last, consider  regions of $\Sigma\setminus(\alphas\cup\betas)$ that have a point $x\in \xxx$ as a corner vertex.  Each such region either has an interval of $\bsGamma$ on its boundary or it has some corner near which it  agrees with one of the thin strips obtained by perturbing the $b_i$ and $b_j^+$ arcs to $a_i$ and $\tilde a_j$ arcs. The positively oriented boundary of such a thin strip near $x$ has a segment of a $\beta$ curve ending at $x$, and a segment of an $\alpha$ curve starting at $x$.  Such a region cannot be in the projection $\pi_{\Sigma}\circ u$ of an index $1$ holomorphic map  
\[u:(S, \bdy S) \to  (\Int(\Sigma)\times \mathbb D \times \R, (\betas\times \{1\}\times \R)\cup (\alphas\times \{0\}\times \R))\]
satisfying \cite[Section 5.2, Conditions (1)-(11)]{bs-JG} and asymptotic to $\xxx\times [0,1]$ at $-\infty$.
Thus, $\delta^1(\xxx_D) = 0$, and $m_{i+1}(\xxx_A, a_1, \ldots, a_i)=0$ for all $i\geq 0$ and all $a_j\in \mathcal A(\bdy \overline{\HH})$.
\end{proof}







 
 
 


==> preliminaries/old/preliminaries.tex <==
% !TEX root = ../bordered-contact-main.tex

\section{Preliminaries}\label{sec:prelim}
This section provides the background required to read the rest of the paper.  We provide references for various classical objects in contact geometry in Section~\ref{ssec:contact} and Heegaard Floer theory in Section \ref{ssec:hf-background}, along with more in-depth summaries of partial open books and the contact invariants in various flavors of Floer homology.  Because we are concerned with the relationships between various theories, we pay particular attention to the conventions for bordered, sutured, and bordered sutured  versions.  Finally, Section~\ref{ssec:afob} gives an efficient introduction to foliated open books.  




\subsection{Assumed background in contact geometry} \label{ssec:contact} Throughout this article, we assume familiarity with many standard definitions in three-dimensional contact geometry, including contact structures; characteristic foliations;  convex surfaces and dividing sets; open book decompositions for closed three-manifolds, as in e.g., \cite{Geiges} and other standard references.  Although we will introduce foliated open books carefully in Section~\ref{ssec:afob} below, we briefly first recall the definition of a partial open book  supporting a contact structure on a manifold with boundary.
\\

\begin{definition}
	A \emph{partial open book} is a triple $(S, P, h)$ where 
	\begin{enumerate}
		\item $S$ is a compact, oriented, connected surface with boundary;
		\item $P$ is a subsurface of $S$ such that the surface $S$ is obtained from $\overline{S\setminus P}$ by successively attaching 1-handles; and
		\item $h \co P\rightarrow S$ is an embedding which is the identity along $\partial P\cap \partial S$.
	\end{enumerate}
\end{definition}


To a partial open book, we can associate a sutured manifold $(M, \Gamma)$, as follows. (See \cite{hkm09} or \cite{EO11} for more details.) Let $H=S\times [-1,0]$ with the identification $(x,t)\sim (x,t')$ for $x\in \partial S$ and $t, t'\in [-1,0]$. Similarly, let $N=P\times [0,1]$ with the identification $(x,t)\sim (x,t')$ for $x\in \partial P\cap \partial S$ and $t, t'\in [0,1]$. Then $M=H\cup N$ where we identify $P\times \{0\}\subset \partial H$ with $P\times \{0\}\subset \partial N$ and $h(P)\times \{-1\}\subset \partial H$ with $P\times \{1\}\subset \partial N$. 
	The suture $\Gamma$ on $\partial M$ can be given as the union of oriented closed curves obtained by gluing the following arcs, modulo identifications:
	$$\Gamma = \overline{\partial S \setminus \partial P}\times \{0\}\cup - \overline{\partial P\setminus \partial S}\times \{1/2\}.$$


\begin{definition}
A contact structure $\xi$ is \emph{compatible} with the partial open book $(S,P,h)$ if for the corresponding sutured manifold $(M=H\cup N, \Gamma)$, the following hold: 

	\begin{enumerate}
		\item $\xi$ is tight on $H$ and $N$;
		\item $\partial H$ is a convex surface in $(M, \xi)$ with dividing set $\partial S\times \{0\}$; and
		\item $\partial N$ is a convex surface in $(M, \xi)$ with dividing set $\partial P\times \{1/2\}$.
	\end{enumerate}
\end{definition}

\subsection{Heegaard Floer theories} \label{ssec:hf-background} We assume familiarity with the various Heegaard Floer theories and provide only a brief review to establish notation and review details related to the contact invariants defined in \cite{oszc, hkm09, HKM09_HF}. 

\subsubsection{Earlier Heegaard Floer theoretic contact invariants}\label{sssec:hfc}

Using open books, Ozsv\'ath and Szab\'o defined a Heegaard Floer  invariant of a closed contact three-manifold \cite{oszc}. For a contact manifold $(M,\xi)$, this invariant is a class $c(\xi)$ in the Heegaard Floer homology $\hfhat(-M)$. 
In \cite{HKM09_HF}, Honda, Kazez, and Mati\'c gave an alternative description of $c(\xi)$. Their construction again uses open books and goes roughly as follows. An open book $(S,h)$ for $(M,\xi)$ induces a Heegaard splitting of $M$ into $U_1\coloneqq S\times \left[0, 1/2\right]$ and $U_2\coloneqq S\times \left[1/2, 1\right]$ with Heegaard surface $\Sigma=(S\times \{1/2\})\cup_B-(S\times\{0\})$. Let $\{a_i\}$ be a collection of properly embedded arcs on $S$ that cut $S$ into a disk.  For all $i$, let $b_i$ be a small perturbation of $a_i$ that moves the endpoints in the positive direction along $\partial S$, so that  $b_i$ intersects $a_i$ in one point.  Fix a basepoint $z$ on $\bdy S$ away from the thin strips cobounded by the $\{a_i\}$ and $\{b_i\}$. It is clear that $\Sigma = \bdy U_1 = -\bdy U_2$,  and that the $\alpha_i := \bdy(a_i\times \left[0,1/2\right])$ bound compressing disks for $U_1$ and the $\beta_i := \bdy(b_i\times \left[1/2,1\right])$ bound compressing disks for $U_2$. Thus, $(\Sigma, \alphas, \betas, z)$ is a Heegaard diagram for $M$. One can see the curves as 
  \begin{align*}
 \alpha_i &= a_i\cup -a_i \subset (S\times \{1/2\})\cup_B-(S\times\{0\}),\\
\beta_i &= b_i\cup -h(b_i) \subset (S\times \{1/2\})\cup_B-(S\times\{0\}).
 \end{align*}
Then 
$c(\xi)\in \hfhat(-M)$
 is defined as the homotopy equivalence class of the unique generator of $\cfhat(\Sigma, \betas, \alphas, z)$ fully supported on $S\times \{1/2\}$.

Using partial open books, Honda, Kazez, and Mati\'c then extended the above construction to define an invariant $EH(M, \Gamma, \xi)$ of contact three-manifolds with convex boundary \cite{hkm09}. In this construction, the roles of $U_1$ and $U_2$ are played by $\big(P\times[-1/2,0]\big)\cup \big(S\times[0,1/2]\big)/\sim$ and $\big(S\times[1/2,1]\big)\cup \big(P\times [-1,-1/2]\big)/\sim$, respectively, and the curves $\{a_i\}$ are the co-cores of the 1-handles $P_i$. The rest of the construction is as above, except that the final generator supported on $P\times \{-1/2\}$ defines an element in the sutured Floer homology $\sfh(-M, -\Gamma)$. Under certain technical conditions, the authors also defined a gluing map for sutured Floer homology that respects the contact invariants  \cite{hkm08}. 



Before briefly reviewing bordered sutured Floer homology, we discuss a straightforward generalization of the contact invariant to multipointed Heegaard diagrams. We begin by constructing a Heegaard diagram analogous to the one above, except that we allow additional arcs $\{a_i\}$ that cut $S$ into $n$ disks. We place a basepoint in each of the disks thus obtained. This results in a multipointed Heegaard diagram $(\Sigma, \alphas, \betas, \mathbf{z})$ for $M$. The unique generator $\mathbf{x}$ on $S\times \{1/2\}$ defines an element in $\HFt(\Sigma, \betas,  \alphas, \mathbf{z}) \cong \hfhat(-M)\otimes H_*(T^{n-1})$. Here $\HFt$ is the homology with respect to the differential that avoids all basepoints, and  $H_*(T^{n-1}) \cong H_*(S^1)^{\otimes(n-1)}$ is the ordinary singular homology of $T^{n-1}$.

An adaptation of the argument of  part (5) of \cite[Theorem 3.1]{BVV} shows the following:
\begin{proposition}\label{lem:multicontact}
Let $(S,h)$ and $(S',h')$ be two open book decompositions compatible with $(M,\xi)$. Let   $\{a_i\}$ and $\{a_i'\}$ be sets of cutting arcs that cut up $S$ and $S'$ into $n$ and $n'$ disks, respectively, with $n<n'$. The graded isomorphism between the Heegaard Floer homologies induced by Heegaard moves, including index $0$ and $3$ stabilizations,  \[
\HFt(\Sigma', \betas',  \alphas', \mathbf{z}') \otimes H_*(T^{n'-n}) \to
\HFt(\Sigma, \betas,  \alphas, \mathbf{z}) \]
 maps the homology class to $[\mathbf{x}'] \otimes \theta^{\otimes{(n'-n)}}$ to $[\mathbf{x}]$, where  $\theta$ corresponds to the lower-degree generator of  $H_*(S^1)$. \qed
\end{proposition}
This means that up to homotopy equivalence, the multipointed contact invariant is simply $c(\xi)\otimes \theta^{\otimes{(n-1)}}$, where $n$ is the number of basepoints. 


We will also make use of the fact that the multipointed Heegaard Floer homology for a closed three-manifold $M$ can be interpreted as the sutured Floer homology of $M$ with balls removed, as follows.
Let $(\Sigma, \alphas, \betas, \mathbf{z})$ be a multipointed Heegaard diagram for  $M$ with $n$ basepoints, and for each basepoint $z\in \mathbf{z}$, let $D^2_z$ be a disk neighborhood of $z$. 
Then $(\Sigma\setminus \cup_\mathbf{z} D^2_z, \alphas, \betas)$ is a sutured Heegaard diagram for  $M(n)  = (M\setminus \cup_{z\in \mathbf{z}}B^3_{z}, \cup_{z\in \mathbf{z}}\partial D^2_z)$. As the two Heegaard diagrams are identical outside the basepointed/sutured regions, the chain complex  $\CFt(\Sigma, \alphas, \betas, \mathbf{z})$ is isomorphic to the chain complex $\SFC(\Sigma\setminus \cup_\mathbf{z} D^2_z, \alphas, \betas)$. Thus, we can compute the multipointed Heegaard Floer homology $\HFt(\Sigma, \betas,  \alphas, \mathbf{z})$ as the sutured Floer homology $\sfh(\Sigma\setminus \cup_\mathbf{z} D^2_z, \alphas, \betas)$. See also \cite[Proposition 9.14]{sfh}. 


\subsubsection{Bordered sutured Floer homology}\label{sssec:bs}

Lipshitz, Oszv{\'a}th, and Thurston refine Heegaard Floer homology to a bordered variant associated to a three-manifold with parametrized boundary \cite{LOTbook, hfmor}, and Zarev \cite{bs, bs-JG} further refines the invariant to an invariant of sutured manifolds with partially parameterized boundary. We briefly discuss Zarev's constructions \cite[Section 3]{bs-JG}. Note that the following description is indicative, rather than complete; for a review of the algebraic definitions involved, see \cite[Section 2]{LOTbook}.

Recall that an \emph{arc diagram} $\mathcal Z = (Z,a,m)$ consists of a finite collection of oriented arcs $Z$, a collection of points $a=(a_1,\cdots, a_{2k})$ on $Z$, a matching $m$ of the points in $a$ into pairs, and a ``type,'' $\alpha$ or $\beta$. To every arc diagram $\zz$ one associates an $\mathcal A_{\infty}$-algebra $\mathcal A(\zz)$ generated by tuples of  oriented arcs in $[0,1]\times Z$  such that each arc connects some $(0,a_i)$ to some $(1, a_j)$ with $a_j\geq a_i$, up to an equivalence relation imposed by the matching. The ground ring of idempotents $\mathcal I(\zz)$ of this algebra consists of elements $\iota$ corresponding to tuples of horizontal strands $[0,1]\times \{a_k\}$ in $[0,1]\times Z$. One further associates to $\zz$ a graph $G(\zz)$ and a surface $F(\zz)$.  The graph is constructed by beginning with $Z$  and adding an edge between each pair of matched points, while  $F(\zz)$ is constructed from $Z \times \left[0,1\right]$ by attaching one-handles to neighborhoods of the matched points on $Z\times \{0\}$. This surface $F(\zz)$ carries sutures $\bsGamma(F) = Z \times \left\{\frac{1}{2}\right\}$.

A bordered sutured manifold $(M,\bsGamma,\zz)$    consists of the following:
\begin{itemize}
\item a three-manifold $M$ whose boundary decomposes as a \emph{bordered} part $F$ and a \emph{sutured} part $T$;
\item an arc diagram $\mathcal{Z}=(Z,a,m)$ and an identification of $F$ with $F(\zz)$;  
\item a decomposition $T=R_+(\bsGamma)\cup R_-(\bsGamma)$ such that $\partial R_{\pm}(\bsGamma)\setminus\bdy F=\pm \bsGamma$. 
\end{itemize}

A $\beta$-bordered Heegaard diagram $\HH=(\Sigma, \alphas, \betas, \zz)$ consists of a compact surface $\Sigma$ with no closed components; a collection of pairwise disjoint, properly embedded circles $\alphas$; a collection of pairwise disjoint, properly embedded circles $\betas^{c}$ and of properly embedded arcs $\betas^{a}$, with $\betas = \betas^a \cup \betas^c$; and an arc diagram $\zz$ of $\beta$-type, together with an embedding $G(\zz)\rightarrow \Sigma$ which maps $Z$ to a subset of $\partial \Sigma$ and the edges of $G(\zz)$ connecting matched points to the arcs $\betas^c$. (An $\alpha$-bordered diagram is defined similarly, mutatis mutandis.) One reconstructs a bordered sutured manifold from $\HH$ by attaching two-handles to $\Sigma\times[0,1]$ along $\alphas \times \{1\}$ and $\betas^c\times \{0\}$ circles. The dividing set $\bsGamma$ appears as $\bsGamma = (\partial \Sigma / Z) \times \left\{\frac{1}{2}\right\}$, and $F(\zz)$ is a neighborhood of $(Z \times [0,1])\cup (\betas^a\times \{0\})$. 


To the Heegaard diagram $\HH=(\Sigma, \alphas, \betas, \zz)$, Zarev associates a left type $D$ module $\bsdhat(\HH)$ and right type $A$ module $\bsahat(\HH)$, both over $\mathcal A(\zz)$. In both cases the generators are as usual tuples of intersection points between the $\alphas$ and $\betas$ such that each $\alpha$-circle is used exactly once and each $\beta$ curve is used no more than once. The type $A$ chain homotopy equivalence class of $\bsahat(\HH)$ is an invariant of $(M, \bsGamma, \zz)$, written $\bsahat(M, \bsGamma, \zz)$. More precisely, given bordered sutured Heegaard diagrams $\HH$ and $\HH'$ for $(M, \bsGamma, \zz)$, there is a sequence of Heegaard moves connecting them as in \cite[Proposition 4.5]{bs}, which induce a type $A$ homotopy equivalence $f$ from $\bsahat(\HH)$ to $\bsahat(\HH')$. This type $A$ homotopy equivalence is a collection of maps
\[f_i:\bsahat(\HH)\otimes \mathcal A(\zz)^{\otimes(i-1)}\to \bsahat(\HH')\]
indexed by $i\ge 1$, satisfying certain conditions (see \cite[Section 2]{LOTbook}). Consider $\x\in\bsahat(\HH)$ and $\x'\in\bsahat(\HH')$ so that 
\[m_{i+1}(\x,a_1,\cdots,a_i)=0\quad\quad\text{and}\quad\quad m_{i+1}(\x',a_1,\cdots,a_i)=0\]
for all $i\ge 0$ and $a_i\in\mathcal{A}(\zz)$. We say $\x$ and $\x'$ are \emph{equivalent} if there exists a homotopy equivalence $f$ from $\bsahat(\HH)$ to $\bsahat(\HH')$ so that $f_1(\x)=\x'$ and $f_{i+1}(\x,a_1,\dots,a_i)=0$ for all $i>0$ and $a_i\in\mathcal{A}(\zz)$. Similarly, there is a type $D$ homotopy equivalence from $\bsdhat(\HH)$ to $\bsdhat(\HH')$. If $\x\in \bsdhat(\HH)$ and $\x'\in\bsdhat(\HH')$ are both closed elements (meaning that $\delta^1(\x)=\delta^1(\x')=0$), we say $\x$ and $\x'$ are \emph{equivalent} if there is a homotopy equivalence from  $\bsdhat(\HH)$ to $\bsdhat(\HH')$ that maps $\x$ to $\x'$.

%A similar statement holds for $\bsdhat(\HH)$ and so it is written as $\bsdhat(M, \bsGamma, \zz)$. 


%To the Heegaard diagram $\HH=(\Sigma, \alphas, \betas, \zz)$, Zarev associates a left type $D$ module $\bsdhat(\HH)$ and right type $A$ module $\bsahat(\HH)$, both over $\mathcal A(\zz)$. In both cases the generators are as usual tuples of intersection points between the $\alphas$ and $\betas$ such that each $\alpha$-circle is used exactly once and each $\beta$ curve is used no more than once. The type $D$ chain homotopy equivalence class of $\bsdhat(\HH)$ is an invariant of $(M, \bsGamma, \zz)$, written $\bsdhat(M, \bsGamma, \zz)$, and similarly for  $\bsahat(M, \bsGamma, \zz)$.

Given two bordered sutured manifolds $(M_i, \bsGamma_i, \zz)$, we may glue along $\zz$ to obtain a sutured manifold $(M, \Gamma)$. Given $\beta$-bordered sutured Heegaard diagrams $\HH_i = (\Sigma_i, \alphas_i, \betas_i, \zz)$ for $(M_i, \bsGamma_i, \zz)$, there is a glued Heegaard diagram $\HH = (\Sigma, \alphas, \betas)$ where $\Sigma = \Sigma_1 \bigcup_{Z} \Sigma_2$; the set $\alphas$ is the union of $\alphas_1$ and $\alphas_2$; and the set $\betas$ is the union of $\betas_1$ and $\betas_2$, together with the circles formed by gluing the arcs in $\betas_1^a$ and $\betas_2^a$ along their endpoints on $Z$.

There is a gluing map
\[
\bsahat(\HH_1) \boxtimes_{\mathcal{A}(\zz)} \bsdhat(\HH_2) \rightarrow SFC(\HH)
\]
which induces a chain homotopy equivalence of vector spaces. Chain homotopy equivalences of type $A$ and type $D$ modules induce chain homotopy equivalences of the box tensor product, so there is a well-defined equivalence class of $\F_2$ vector spaces $\bsahat(M_1, \bsGamma_1, \zz) \boxtimes_{\mathcal{A}(\zz)} \bsdhat(M_2, \bsGamma_2, \zz)$, and an equivalence of chain homotopy equivalence classes of vector spaces
\[
\bsahat(M_1, \bsGamma_1, \zz) \boxtimes_{\mathcal{A}(\zz)} \bsdhat(M_2, \bsGamma_2, \zz) \rightarrow SFC(M, \Gamma).
\]

\subsection{Abstract foliated open books}\label{ssec:afob}


In this section, we provide an  overview of the essential definitions and properties of foliated open books that we will rely on in the remainder of this article.   Readers are encouraged to see \cite{LV} for more detail.


\begin{definition}\cite[Definition 3.12]{LV}\label{def:afob} An \emph{abstract foliated open book} is a tuple $(\{S_i\}_{i=0}^{2k}, h)$ where $S_i$ is a surface with 
boundary $\partial S_i=B\cup A_i$ \footnote{By a slight abuse of notation we denote the ``constant" part of the boundary of $S_i$ by $B$ for all $i$.} and corners at $E=B\cap A_i$ such that 
\begin{enumerate}
\item for all $i$, $A_i$ is a union of intervals;
\item with the boundary orientation, each component $I$ of $A_i$ is oriented from a corner labeled $e_+ = e_+(I)\in E_+$ to a corner labeled $e_- = e_-(I)\in E_-$, and $E=E_+\cup E_-$;

\item the surface $S_{i}$ is obtained from $S_{i-1}$ by either 
\begin{itemize}
\item[-]\textbf{(add):} attaching a 1-handle along two points $\{p_{i-1}, q_{i-1}\}\in A_{i-1}$, or 
\item[-]\textbf{(cut):} cutting $S_{i-1}$ along a properly embedded arc $\gamma_{{i}}$ with endpoints in $A_{{i-1}}$ and then smoothing.\footnote{The indices of $\gamma_i$ in this paper are shifted compared to \cite{LV}, where the cutting arcs were denoted by $\gamma_{i-1}$.}
\end{itemize}
\end{enumerate}

Furthermore,  $h \colon S_{2k}\rightarrow S_0$ is a diffeomorphism between cornered surfaces that
preserves $B$ pointwise. 
\end{definition}
We denote by $H_+$ (resp.~$H_-$) the set of indices $i$ for which $S_{i}$ is obtained from $S_{i-1}$ by cutting  (resp.~adding), so that we have a partition $[2k]=H_+\cup H_-$. 


Note that the operations \textbf{(add)} and \textbf{(cut)} are  inverses  of each other.  Let $\gamma$ denote the cocore of a handle attached along points $p$ and $q$.  Then cutting along $\gamma$ cancels the handle attachment, and vice versa. We will use the following notation to describe this:
\[S\xrightarrow[{p,q}]{\text{\textbf{add}}} S' \text{    and    } S'\xrightarrow[{\gamma}]{\text{\textbf{cut}}}S.\] 

\begin{example}\label{ex:torus}
Figure~\ref{fig:afobtorus} shows a first example of a foliated open book.  The complete set of labels is shown for the indicative page $S_0$, while the attaching spheres and cutting arcs are shown on all pages to the right.  The binding is shown in bold. The monodromy $h \colon S_4\rightarrow S_0$ is the identity, and we have the partition $H_-=\{2,4\}$, $H_+=\{1, 3\}$. 
\begin{figure}[h]
\begin{center}
\includegraphics[scale=1]{preliminaries/afobtorusshiftL}
\caption{A foliated open book with $k=2$.}\label{fig:afobtorus}
\end{center}
\end{figure}
\end{example}


\subsubsection{Supported contact structures}
\label{sec:supp-cs}


The construction of a compact manifold is natural from the data of a foliated open book: pairs of successive pages define cornered cobordisms.  As described in more detail below, we concatenate these to form a manifold with boundary and collapse the resulting components of $B\times I$ to circles and intervals again labeled $B$.  The final page glues to the initial page via $h$. The resulting  manifold $M$ associated to the foliated open book $(\{S_i\}_{i=0}^{2k}, h)$ retains partial information about the sequence of cuts and adds in the abstract data. This information is encoded in the form of boundary decorations on $\partial M$, and we introduce the kind of foliation we will consider before explaining how it arises:

\begin{definition}  A \emph{signed singular foliation} is an equivalence class of smooth vector fields that vanish at only finitely many isolated points, called \emph{singular points}. The  complement of the singular points has an open cover such that in each ball, the integral curves of the vector field are a product of oriented intervals, while elliptic and four-pronged hyperbolic singularities patch these charts together. Elliptic singularities may be classified as positive (sources) or negative (sinks), and the hyperbolic singularities have signs determined by input external to the defining vector field.  
\end{definition}
 
 See Figure \ref{fig:sing} for local models of the integral curves.
% \emph{signed singular foliation}.  In the complement of finitely many isolated singular points, a signed singular foliation is an equivalence class of smooth non-vanishing vector fields whose integral curves decompose an open set in $\partial M$ as a product of  intervals, while elliptic and four-pronged hyperbolic singularities are allowed in order to patch this open cover together, as in Figure \ref{fig:sing}. Elliptic singularities may be classified as positive (sources) or negative (sinks), while the signs on hyperbolic singularities require input external to the defining vector field. The leaves that enter (or exit) the hyperbolic singularities are called \emph{stable (or unstable) separatrices}.   

As is  standard, leaves that enter (or exit) the hyperbolic singularities are called \emph{stable (or unstable) separatrices}.   

\begin{figure}[h]
\begin{center}
\includegraphics[scale=.8]{preliminaries/sing}
\caption{Left: a hyperbolic singularity.  Center: a positive elliptic singularity. Right: a regular foliation on an open set.}\label{fig:sing}
\end{center}
\end{figure}
  
Beginning with an abstract foliated open book, we now build a manifold whose boundary is naturally equipped with a  signed singular foliation. Each pair of successive pages defines an elementary cobordism $M_i$
from $S_{i-1}$ to $S_{i}$ with vertical boundary $(B\times I)\cup V_i$, where $V_i$ is the union of a single saddle and of the collection of products $A_{i-1}\times I$ for any components $A_{i-1}$ that are left unchanged.  More specifically, the saddle connects either the components of $A_{i-1}$ containing the endpoints of $\gamma_{i}$  or the component(s) containing $p_{i-1}$ and $q_{i-1}$ with the  obtained component(s) of $A_i$ that have the same endpoints. See Figure~\ref{fig:cobord}. 

\begin{figure}[h]
\begin{center}
\includegraphics[scale=.6]{preliminaries/cobordL}
\caption{The elementary cobordism associated to cutting $S_{i-1}$ along $\gamma_i$, shown before collapsing $B\times I$.}\label{fig:cobord}
\end{center}
\end{figure}


Concatenating these $M_i$ and gluing the final $S_{2k}$ to the initial $S_0$ via $h$ yields a manifold with boundary $(B\times S^1) \cup V$, where $V$ is the (circular) union of the $V_i$.  The singular foliation on $V$ has $2k$ singular points  associated to the transitions between topological types of the pages, while the regular leaves may be identified with curves of the form $A_i\times \{t\}$. 
If $S_{i-1}\xrightarrow{\text{\textbf{add}}} S_{i}$, then the corresponding hyperbolic point $h_i$ is negative; otherwise, it is positive. We denote the set of hyperbolic points with respect to this 
partition $H=H_+\cup H_-$. The signs match the partition of $[2k]$ introduced after Definition~\ref{def:afob}.
 Collapsing the components $B\times S^1$ to a single copy of $B$ yields a manifold with foliated boundary, a  term we will define precisely in Definition~\ref{def:mfb} $(M, \partial M, \mathcal{F})$.   Each endpoint  of $B$ labeled $e_+$ becomes a positive elliptic point of the foliation, which we again denote by $e_+$; likewise, an endpoint $e_-$ becomes a negative elliptic point $e_-$.  
 
 \begin{example} We return to the foliated open book introduced in the first example. The associated smooth manifold is the solid torus shown in Figure~\ref{fig:afobtorusmfd}. The images of $A_1$ and $A_2$ are shown in green and blue, respectively, on both the manifold on the left and in the associated boundary foliation on the right.
 


\begin{figure}[h]
\begin{center}
\includegraphics[scale=1]{preliminaries/afobtorusmfdL}
\caption{The smooth manifold (a solid torus) associated to the  foliated open book from Figure~\ref{fig:afobtorus}  together with the foliation $\mathcal{F}$ on $\partial M$.}\label{fig:afobtorusmfd}
\end{center}
\end{figure}
\end{example}
 
 
 In order to define the compatibility between contact structures and foliated open books, we  examine the boundary foliation $\mathcal{F}$ more closely.  To any smooth manifold constructed  as above, we may associate  an  $S^1$-valued regular function $\pi \colon  M \setminus B \rightarrow S^1$  whose level sets are the pages of the open book and which restricts to the boundary as an $S^1$-valued Morse function $\pit:=\pi|_{\partial M}\colon \partial M\setminus E\to S^1$. 
 One may build a signed singular foliation simply by patching together the local models of Figure~\ref{fig:sing}, but in the context of this paper we will only encounter  signed singular foliations which can be induced by such an $S^1$-valued Morse function.  We therefore consider the map $\pit$ to be an essential part of the data and we write  $\fol=(\pit, H=H_-\cup H_+, E=E_-\cup E_+)$.  We may also assume that $0$ is a regular value of $\pi$ and we further require that $\pit=\pm\phi$ on an $(r, \phi)$-disk neighborhood of each elliptic point $e\in E$, where the sign depends on the sign of the elliptic point. Here $(r,\phi)$ is the standard polar coordinate system on $D^2$.   By construction, the foliation on a manifold constructed from an abstract foliated open book has only elliptic and four-pronged hyperbolic singularities, with  signs inherited from the  partitions of $E$ and $H$.  
  
  
 \begin{definition}\label{def:mfb}
 A \emph{manifold with foliated boundary}  is a compact oriented three-manifold equipped with a signed singular foliation $\fol=(\pit, H=H_-\cup H_+, E=E_-\cup E_+)$ on its boundary. We denote this collection of data by  $(M, \partial M, \mathcal{F})$. %\vv{A \emph{diffeomorphism} between manifolds with foliated boundary are required to bring the foliations together with the corresponding $S^1$-valued functions to each other.}
 \end{definition}
  
   We recall  that this data includes the $S^1$-valued Morse function $\pit$, and we  %, and that the upcoming construction will  depend heavily on $\pit$. 
  require that a diffeomorphism $f:(M_1, \partial M_1, \fol_1) \rightarrow (M_2, \partial M_2, \fol_2)$  between manifolds with foliated boundary must satisfy $\pit_2\circ f= \pit_1$.
   
 We have seen that an abstract foliated open book gives rise to a diffeomorphism class of manifolds with foliated boundary; we say a manifold with foliated boundary is \emph{compatible} with $(\{S_i\}, h)$ if it is diffeomorphic to an output of this construction. A fixed manifold with foliated boundary will admit many different functions $\pi$ extending the Morse function $\pit$ on the boundary, but compatibility identifies an equivalence class of such functions whose level sets are diffeomorphic to the pages $\{S_i\}$. 
 % \marginpar{\vv{OK, not 100 percent precise, but understandable, to make it precise it has to be made longer, so I am OK.}}
 
  \begin{definition}\label{def:div} Suppose that $\fol=(\pit, H=H_-\cup H_+, E=E_-\cup E_+)$ is a signed singular foliation with no $S^1$ leaves.  We define $R_+(\fol)$ to be a closed neighborhood of the union of the stable separatrices of hyperbolic points in $H_+$, and let $R_-(\fol)=\overline{M\setminus R_+(\fol)}$. 
  The \emph{dividing curve} $\Gamma(\fol)$ of $\fol$ is  $\partial R_+(\fol)=-\partial R_-(\fol)$.
  \end{definition} 
  
Note that $\Gamma$ is distinct from the $\bsGamma$ introduced in Section~\ref{sssec:bs} as part of the defining data of a bordered sutured manifold, and further, that $\Gamma(\fol)$ indeed divides $\fol$: $\Gamma(\fol)$ is positively transverse to the leaves of $\fol$ and it separates $\partial M\setminus \Gamma(\fol)$  into two parts, one of which contains all the positive singular points, while the other part contains all the negative singular points.\footnote{Readers concerned that we have not addressed a third condition associated with dividing curves in contact geometry are referred to Lemma 2.6 of \cite{LV}.} These  properties in fact specify $\Gamma(\fol)$ up to isotopy transverse to $\fol$, and we will often work with its equivalence class, only specifying the specific representative when needed. The choice of the representative then changes $R_+(\fol)$ and $R_-(\fol)$ accordingly, while still preserving the condition that $\Gamma(\fol)=\partial R_+(\fol)=-\partial R_-(\fol)$.   Note that distinct foliations on $\partial M$ may induce isotopic dividing sets; see Figure~\ref{fig:folball}.

 
 

  
   \begin{definition}
   Two signed singular foliations $\fol_1$ and $\fol_2$ on a surface $\Sigma$ are \emph{strongly topologically conjugate} if 
	\begin{itemize}
	\item there is a multicurve $\Gamma$ which divides both $\fol_1$ and $\fol_2$, and
	\item there is an isotopy taking $\fol_1$ to $\fol_2$ which preserves $\Gamma$ setwise.
   \end{itemize}
   \end{definition}
   
 The term ``topological'' refers to the fact that the above isotopy may not be smooth. In fact, in the next definition, the isotopy cannot be chosen to be smooth.  
 
    
% \vv{ \begin{definition} \cite[Definition 3.7]{LV} A contact structure $\xi$ on a manifold with foliated boundary  $(M, \partial M, \mathcal{F})$ is \emph{supported by} (or \emph{compatible with}) the abstract foliated open book $(\{S_i\}, h)$ if   $(M, \partial M, \mathcal{F})$ is diffeomorphic to the manifold with foliated boundary constructed for the abstract foliated open book $(\{S_i\}, h)$ as above, and for the pull-back of some contact form we have:
% \begin{enumerate}
 %\item $\alpha(TB)>0$;
 %\item for all $t$, $d\alpha|_{\pi^{-1}(t)}$ is an area form; and
 %\item $\mathcal{F}$ is strongly topologically conjugate to the characteristic foliation $\mathcal{F}_{\xi}$.
 %\end{enumerate}
 %\end{definition} }
 
% \marginpar{\vv{I like the version of the definition before (put it back in blue). I think you cannot start talking about a contact structure before you fix the manifold.. I was trying to fix the order, and then I got back to the old version. What's wrong with it?}}
 
% \ip{They both have imprecisions to me. Can I suggest a third version? Note that sentences are too long in each version, so we're not winning awards for style, but I think teal is about right. Blue wasn't clear on what's being pulled back from where to where, and in red the manifold for $\xi$ was missing. I just noticed that in red the manifold is "compatible with" the AFOB, so technically it's only \emph{diffeomorphic to} one constructed from the AFOB, so we can't talk about "pages" as subsets of it, and we don't have a function $\pi$ on $M$. I think the teal writeup actually incorporates Vera's margin remarks a few lines below. }
 
 \begin{definition} \cite[Definition 3.7]{LV} A contact structure $\xi$ on a manifold with foliated boundary  $(M, \partial M, \mathcal{F})$ is \emph{supported by}  the abstract foliated open book $(\{S_i\}, h)$    if  there is a diffeomorphism $f\colon (M', \partial M', \mathcal{F'})\to (M, \partial M, \mathcal{F})$, where $(M', \partial M', \mathcal{F'})$ is a manifold constructed from $(\{S_i\}, h)$ as above, such that the pullback $f^{\ast}\xi$ is the kernel of some one-form $\alpha$ on $M'$ satisfying the following conditions:
 \begin{enumerate}
 \item $\alpha(TB)>0$;
 \item for all $t$, $d\alpha|_{\pi^{-1}(t)}$ is an area form; and
 \item $\mathcal{F}$ is strongly topologically conjugate to the characteristic foliation $\mathcal{F}_{\xi}$.
 \end{enumerate}
 \end{definition} 
 
 % \jel{ \begin{definition} \cite[Definition 3.7]{LV} The contact structure $\xi$ is  \emph{supported by} the abstract foliated open book $(\{S_i\}, h)$ if there exists a manifold with foliated boundary $(M ,\partial M, \fol)$ compatible with $(\{S_i\}, h)$ with a contact form $\alpha$ such that  the following conditions hold:
 %\begin{enumerate}
 %\item $\xi=\ker \alpha$;
 %\item $\alpha(TB)>0$;
 %\item for all $t$, $d\alpha|_{\pi^{-1}(t)}$ is an area form; and
 %\item $\mathcal{F}$ is strongly topologically conjugate to the characteristic foliation $\mathcal{F}_{\xi}$.
 %\end{enumerate}
 %\end{definition} }



% \jel{ \begin{definition} \cite[Definition 3.7]{LV} Fix an abstract open book and suppose that $(M, \partial M, \mathcal{F})$ is  a manifold with foliated boundary constructed from $(\{S_i\}, h)$  as above.  Then the contact structure $\xi$ is \emph{supported by} $(\{S_i\}, h)$ if  $\xi=\ker \alpha$ for a contact form satisfying the following conditions on $(M, \partial M, \mathcal{F})$:
% \begin{enumerate}
% \item $\alpha(TB)>0$;
% \item for all $t$, $d\alpha|_{\pi^{-1}(t)}$ is an area form; and
% \item $\mathcal{F}$ is strongly topologically conjugate to the characteristic foliation $\mathcal{F}_{\xi}$.
% \end{enumerate}
% \end{definition} }

%\jel{We will also say that $\xi$ is compatible with $(\{S_i\}, h)$.}\marginpar{\jel{Preferably, we would choose one phrase and use it consistently. }}
   
   
% \begin{definition} \cite[Definition 3.7]{LV} The abstract foliated open book $(\{S_i\}, h)$ \emph{supports} the contact structure $\xi$ on $(M, \partial M, \mathcal{F})$ if $\xi$ is the kernel of some one-form $\alpha$ on $M$ satisfying the following properties:
% \begin{enumerate}
 %\item $\alpha(TB)>0$;
 %\item for all $t$, $d\alpha|_{\pi^{-1}(t)}$ is an area form; and
 %\item $\mathcal{F}$ is strongly topologically conjugate to the characteristic foliation $\mathcal{F}_{\xi}$.
% \end{enumerate}
 %\end{definition} 



\begin{definition}\label{def:mxif} A \emph{foliated contact three-manifold} $(M, \xi, \fol)$ is a manifold with foliated boundary together with a contact structure $\xi$ on $M$ such that $\fol$ is strongly topologically conjugate to $\mathcal{F}_{\xi}$.  \end{definition} 




\begin{theorem}\cite[Theorems 3.10, 7.1, 7.2]{LV} \label{thm:support}
Any foliated open book supports a unique isotopy class of contact structures, and any foliated contact three-manifold $(M,\xi,\mathcal{F})$ admits a supporting foliated open book.
\end{theorem}


%\marginpar{\jel{*can we really talk about an isotopy class of contact structures on a manifold defined up to diffeomorphism?*} \vv{I think it's OK. But we have to be careful how we phrase it. We first fix the manifold, with a supporting abstract FOB, this gives a diffeo $\phi: M\to M'$, where $M'$ is the "ideal" (in the sense of Plato) manifold constructed from the abstract FOB.  And there is up to isotopy unique contact structure on $M'$, and the diffeo $\phi$ can also be changed by conjugating by isotopies (well, that'd be the statement, I am not sure we proved this in our case).}}


%\vv{As customary, we only work up to contactomorphism, and say that a  foliated contact three-manifold $(M, \xi, \fol)$ is \emph{supported} by an abstract open book $(\{S_i\}_{i=0}^{2k}, h)$ if it is contactomorphic to the foliated contact three-manifold constructed from $(\{S_i\}_{i=0}^{2k}, h)$ as above.}
%\vv{\begin{theorem}\cite[Theorems 7.1, 7.2]{LV} \label{thm:support2}
%Any foliated contact three-manifold $(M,\xi,\mathcal{F})$ admits a supporting foliated open book.
%\end{theorem}}



\begin{remark}\label{rmk:t} Because the  signed singular foliation $\fol$ data includes a function $\widetilde{\pi}$, a foliated contact three-manifold has a distinguished $t=0$ leaf, which we always assume to be regular.  
\end{remark}

Distinct foliations may  induce isotopic dividing sets, as illustrated in the following example. 

\begin{example} Let $(B^3, \xi_1, \fol_1)$ and $(B^3, \xi_2, \fol_2)$ be two foliated contact three-balls with $\xi_1$ and $\xi_2$ tight, and with the foliations $\fol_1$ and $\fol_2$ on the boundaries as in Figure~\ref{fig:folball}. Although the two three-balls are contactomorphic, these are distinct as foliated contact manifolds.


\begin{figure}[h]
\begin{center}
\includegraphics[scale=1]{preliminaries/folballL}
\caption{Left: A foliation on $S^2$ with four elliptic points and two hyperbolic points. Right: A foliation on $S^2$ with two elliptic points. The dividing set for each foliation is a circle. }\label{fig:folball}
\end{center}
\end{figure}
\end{example}


\subsubsection{Stabilization}

Although each foliated open book supports a unique isotopy class of contact structures, there are many foliated open books which support the same class.  Next, we define an operation which changes a foliated open book while preserving the contactomorphism class of the associated contact manifold.  

\begin{definition}\label{def:stab} Let $\gamma\subset S_0$ be a properly embedded arc with $\partial \gamma\subset B$.  The \emph{stabilization of $(\{S_i\}, h)$ along $\gamma$} is the foliated open book $(\{S'_i\}, h')$ defined as follows:
\begin{itemize}
\item $S_i'=S_i\cup H$, where $H$ is a one-handle attached along $\partial \gamma$; and 
\item $h'=\tau \circ \overline{h}$, where $\tau$ is a positive Dehn twist along the circle formed by $\gamma$ and the core of $H$. (Here $\overline{h}$ denotes the extension of $h$ to $H$ by the identity.) 
\end{itemize}
\end{definition}


In order to define stabilization along some arc in a page besides $S_0$, we first describe an operation on foliated books which preserves the contactomorphism type of the associated manifold.
\begin{definition}\cite[Definition 3.14]{LV}
The $1$-\emph{shift} of an abstract foliated open book $(\{S_i\}_{i=0}^{2k},h)$ is the foliated open book \[(\{S_i[1]\}_{i=0}^{2k},h[1])=(\{S_1,S_2,\dots,S_{2k},S_1'\},h'),\] where

\begin{itemize}
\item[-] if $S_{0}\xrightarrow[\gamma_{1}]{\text{\textbf{cut}}} S_1$, then $S_1'$ is defined by the relation $S_{2k}\xrightarrow[{h^{-1}(\gamma_{1})}]{\text{\textbf{cut}}} S_1'$ and $h'$ is the restriction of $h$  to $S_1'$;
\item[-] if $S_{0}\xrightarrow[{p_0, q_0}]{\text{\textbf{add}}} S_1$, then $S_1'$ is defined by the relation $S_{2k}\xrightarrow[{ h^{-1}(p_0), h^{-1}(q_0) }]{\text{\textbf{add}}} S_1'$ and $h'$ is $h$ extended by the identity on the added 1-handle. 
\end{itemize}
An $r$-fold iteration of the shift operation is called an \textit{$r$-shift}, and denoted by $(\{S_i[r]\}_{i=0}^{2k},h[r])$. One can analogously define $r$-shifts for $r<0$.
\end{definition}
Shifts correspond to post-composing $\pi$ with a diffeomorphism of $S^1$.

\begin{definition}
Let $\gamma\subset S_r$ be a properly embedded arc with $\partial \gamma\subset B$. The stabilization of $(\{S_i\}, h)$ along $\gamma\subset S_r$ is the foliated open book $(\{S'_i\}, h')$ defined as follows:

\begin{enumerate}
\item first perform an  $r$-shift of $(\{S_i\},h)$ to $(\{S_i[r]\},h[r])$;
\item\label{item:handle}   stabilize as in Definition~\ref{def:stab} along the image of $\gamma\subset S_r[r]$;
 \item perform a $(-r)$-shift  to obtain $(\{S_i'\},h')$, where  $S_i'$ is still obtained from $S_i$ by a handle attachment along $p$ and $q$.
 \end{enumerate}
\end{definition}

It is easy to see that stabilizing does not change the underlying manifold with foliated boundary.

\begin{theorem}\cite[Proposition 6.8, Theorem 6.9]{LV}\label{thm:supportstab}
Let $(\{S_i\}, h)$ be a foliated open book and $(\{S_i'\}, h')$ be a positive stabilization of $(\{S_i\}, h)$. Then the corresponding contact three-manifolds are contactomorphic. Furthermore, if two foliated open books support contactomorphic foliated contact three-manifolds, then they admit a common positive stabilization. \end{theorem}







\subsubsection{Sorted foliated open books}

Next, we introduce some additional bookkeeping  to record the cutting arcs and cocore arcs on all possible pages of the foliated open book.  This additional information corresponds to a choice of a gradient-like vector field on the associated smooth manifold, as we will describe in Section~\ref{sec:morse}. 

If $S_{{i-1}}\xrightarrow{\text{\textbf{add}}} S_{i}$, then for all $j\geq {i}$, decorate $S_{j}$ with a cocore of the added handle and label this cocore $\gamma_i^-$. If $S_{{i-1}}\xrightarrow{\text{\textbf{cut}}} S_{i}$ along $\gamma\subset S_{{i-1}}$, then for all $j\leq {i-1}$, decorate $S_j$ with the cutting curve and label it $\gamma_i^+$. 

We call the  $\gamma_i^\pm$ \emph{sorting arcs}. Note that by an abuse of notation we use a single label $\gamma_i^\pm$ to refer to distinct copies of the sorting arcs on multiple $S_j$.  In general, sorting arcs may intersect (and consequently some sorting arcs may appear as a union of disconnected intervals on some pages). We will shortly restrict to the subclass of \emph{sorted} foliated open books \cite[Section 5.3]{LV}, which  are characterized by the requirement that the sorting arcs are disjoint on all pages, together with a prescribed ordering of the intersections between sorting arcs and regular leaves.  In the sorted case, we enhance the notation for describing a foliated open book to reflect these additional choices:




\begin{definition}\label{def:sorted}An abstract foliated open book $(\{S_i\}, h, \{\gamma_i^\pm\})$ is \emph{sorted} if  the following properties hold: 
\begin{enumerate}
  \item\label{item:pm}  on each page $S_i$ and for each component $I$ of $A_i$ with $\partial I=\{e_+, e_-\}$, there exist disjoint subintervals  $I_+$ and $I_-$  such that $I_+$ contains $e_+\cup \bigcup_j \big(\gamma^+_j\cap I\big)$ and  $I_{-}$ contains $e_-\cup \bigcup_j \big(\gamma^-_j\cap I\big)$.
 
\item\label{item:plus} for $i {<} j<k$, on each component of $A_i$ any endpoint of $\gamma_k^+$ is closer to $e_+$ than any endpoint of $\gamma_j^+ $;


\item\label{item:minus} for $j<k\leq i$, on each component of $A_i$ any endpoint of $\gamma_k^-$  lies closer to $e_+$ than any endpoint of $\gamma_j^-$; 

\item on each page, the sorting arcs are connected, properly embedded, and disjoint. 
\end{enumerate}
\end{definition}

See Figure~\ref{fig:sorttorus} in Example~\ref{ex:sorted} for an illustration of the ordering conventions given above.
 Sorted foliated open books are useful  because of their close relation to partial open books, which will be described in Section~\ref{sssec:suff}. Below, we show that a foliated open book need not be sorted. 
 




\begin{example}
The foliated open book from Example~\ref{ex:torus} is not sorted.  To see this, we start on the $S_0$ page and attempt to decorate each successive page with cutting arcs which realize the topological transitions between pages and whose endpoints also satisfy the ordering conditions of Definition~\ref{def:sorted}. 

Cutting along $\gamma_1^+$ on $S_0$ yields $S_1$, while attaching a handle to $S_1$ gives rise to $S_2$, which is decorated with the new cocore $\gamma_2^-$.  However, any cutting arc associated to $h_3$ necessarily intersects $\gamma_2^-$ on $S_2$, as the endpoints of $\gamma_3^+$ must lie closer to the positive ends of $A_2$ than the endpoints of $\gamma_2^-$.  Thus the foliated open book is not sorted. 
\begin{figure}[h]
\begin{center}
\includegraphics[scale=1]{preliminaries/efobtorusnotsortedL}
\caption{The first three pages of the foliated open book from Example~\ref{ex:torus}.}\label{fig:orderofseps}
\end{center}
\end{figure}
\end{example}


We may always stabilize a foliated open book to obtain a sorted one. 
\begin{theorem} \label{thm:revsortedsupport} 
Any foliated contact three-manifold $(M,\xi,\mathcal{F})$ admits a supporting sorted foliated open book. Moreover, if two sorted foliated open books support the same foliated contact three-manifold, then we can stabilize each through sorted foliated open books to obtain a common sorted foliated open book. Moreover, all of these stabilizations can be assumed to be performed on the $S_0$ page  
as in Definition \ref{def:stab}.
\end{theorem}

\begin{proof} The first two statements are taken from \cite [Theorem 3.10, Theorem 8.14]{LV}. The final claim that the necessary stabilisations may be assumed to occur on the $S_0$ page is implicit in \cite{LV}, as explained next; we include the brief argument here, although it relies on the connection between foliated and partial open books described in Section~\ref{sssec:suff}.  Specifically, the proof of \cite[Proposition 8.6]{LV}  explains why stabilizations on the $S_0$ page suffice to turn an arbitrary  sorted foliated open book into a sufficiently stabilized\footnote{This subclass consists of the foliated open books which can most easily be related to partial open books, a relationship which we discuss shortly.} foliated open book.    The proof that two sufficiently stabilized open books admit a common stabilization relies on Giroux Correspondence for the associated partial open books, and hence, leads again to stabilizations on $S_0$. 
\end{proof}

\begin{example}\label{ex:sorted}
Figure~\ref{fig:sorttorus} shows that the foliated open book from Example~\ref{ex:torus} may be stabilized to a sorted foliated open book.  Starting from index $S_0$, the first obstruction to being sorted occurred as an intersection between $\gamma_2^-$ and $\gamma_3^+$ on $S_2$.   This intersection may be removed by stabilizing ``at'' the $S_2$ page; that is,  by shifting twice and then stabilizing at the new $S_0$. Each new page is obtained from the corresponding old page by attaching a one-handle with one attaching interval on each binding component.  The new final maps to the new initial page by a positive Dehn twist; after shifting back, this becomes a positive Dehn twist identifying the two copies of the $S_2'$  page, as shown.  Thus  $\gamma_2^-$ changes by a positive Dehn twist as it ascends to higher-index pages, while  $\gamma_3^+$ changes by a negative Dehn twist as it descends to lower-index pages.  

\begin{figure}[h]
\begin{center}
\includegraphics[scale=1]{preliminaries/efobtorusstab2L} 
\caption{The stabilization arc $\gamma\subset S_0$ is chosen to have one endpoint on each interval of the binding $B$ so that it crosses each of of the intersecting sorting arcs in Figure~\ref{fig:orderofseps} exactly once.  There is a right-handed Dehn twist identifying the two copies of the $S_2'$ page, while the monodromy $h' \co S_4'\to S_0'$ is translation in the plane of the page. The sorting arcs $\gamma^+$ are shown in light blue, and the sorting arcs $\gamma^-$ are shown in dark blue. Subintervals $I_\pm\subset A_0$ are highlighted in green and orange on $S_0$ and may be chosen analogously on the other pages.}\label{fig:sorttorus}
\end{center}
\end{figure}

When depicting a sequence of pages, there is an implicit identification by translation in the page unless otherwise noted.  In this example, the one non-translation occurs at $S_2'$ while the map from $S'_4$ to $S_0'$ remains  translation in the plane of the page, as seen on Figure~\ref{fig:sorttorus}.  The result is a sorted foliated open book for the original contact manifold with foliated boundary.  
\end{example}






\subsubsection{Gradient flows on foliated open books}\label{sec:morse}

As in Section~\ref{sec:supp-cs}, we consider the smooth manifold with foliated boundary $(M, \partial M, \mathcal{F})$ constructed from a foliated open book. The initial abstract data determines an equivalence class of circle-valued Morse functions $\pi \co M\setminus B\rightarrow S^1$ \cite[Section 5.2]{LV}.  The level sets of $\pi$ are the pages, and the restriction $\pit \co \partial M\setminus B \rightarrow S^1$ is again a circle-valued Morse function with the same set of critical points.  In this setting, one may consider the critical submanifolds of the gradient-like vector field.  The intersection of the critical submanifolds with the regular level sets of $\pi$ determines sorting arcs on the pages of the corresponding abstract foliated open book \cite[Section 5.3]{LV}. Thus a foliated open book is sorted when a gradient-like vector field on $\partial M$ that satisfies the ordering conditions for sorting arcs extends to a gradient-like vector field on $M$ whose critical submanifolds are disjoint. 

Any surface with an open book foliation decomposes along regular leaves into square tiles that each contain precisely one hyperbolic singularity.  Figure~\ref{fig:rgradient} shows the flowlines of  a preferred $\nabla \pit$ on such a tile; these flowlines satisfy the ordering conditions in Definition~\ref{def:sorted}, although ensuring their extension to $M$ yields a sorted foliated open book may require stabilization.  

\begin{figure}[h]
\begin{center}
\includegraphics[scale=.65]{preliminaries/gradientcorrectL}
\caption{The tile of $\fol$ shows  purple flowlines of $\nabla \pit$ which satisfy the sorted ordering conditions.}\label{fig:rgradient}
\end{center}
\end{figure}

The Morse perspective is useful not only for building geometric intuition, but also for relating the boundary decorations to those in the interior of the manifold.  For example, a sorting arc $\gamma^\pm_i$ is isotopic through the associated (un)stable critical submanifold of $\nabla\pi$ to the (un)stable submanifold of $\nabla\pit$ on $\partial M$ which passes through 
the corresponding positive (negative) hyperbolic point $h_i$.
  Conditions~\ref{item:pm}, \ref{item:plus}, and \ref{item:minus} in Definition~\ref{def:sorted} are chosen so that the graphs formed by  the (un)stable separatrices of positive (negative) hyperbolic points with respect to $\fol$ and with respect to $\nabla \pit$ are isotopic.  In the next section, this will allow us to define certain subsurfaces as neighborhoods of either graph. 

\subsubsection{Sufficiently stabilized foliated open books and the  associated partial open book} \label{sssec:suff}


Sorted foliated open books are closely related to partial open books, and \cite{LV} introduced the technical designation of a ``sufficiently stabilized" foliated open book. In this section, we recall this definition and show that a sufficiently stabilized foliated open book naturally has a companion partial open book.  Throughout this section, we will let $(\{S_i\}_{i=0}^{2k},h,\{\gamma_i^\pm\})$ be a sorted foliated open book and $(M, \xi, \fol)$ be the supported foliated contact three-manifold.  We further assume that either $k>0$ or $|\partial M|>1$; the only foliated open books this excludes are those formed from an honest open book by removing a neighborhood of a single point on the binding.

Set
\[R_i=N_{\lrcorner}\big(A_i \cup(\bigcup_{i < j}\gamma_j^+)\cup(\bigcup_{i\geq j}\gamma_j^-)\big) \subset S_i,\]
 where $N_{\lrcorner}$ denotes a ``cornered'' neighborhood of $A_i \cup(\bigcup_{i < j}\gamma_j^+)\cup(\bigcup_{i\geq j}\gamma_j^-)$, with corners at $E$, so that $R_i$ meets $B$ only at $E$.  
Furthermore, define \[P_i=\overline{S_i\setminus R_i},\]
as shown on the left in Figure~\ref{fig:sssorttorus}.
Since only the $R_i$  change with $i$, we can identify all the $P_i$ with each other by the flow of the gradient-like vector field. {We denote the composition of these identifications from $P_0\subset S_0$ onto $P_{2k}\subset S_{2k}$ by $\iota$}.  
{Let $\widetilde{S}=S_{0}$, $\widetilde{P}=P_{0}$ and $\tilde{h}=h\vert_{P_{2k}}\circ \iota$}. 


\begin{definition}\cite[Proof of Proposition 8.6]{LV} The sorted foliated open book $(\{S_i\}_{i=0}^{2k}, h, \{\gamma_i\})$ is \emph{sufficiently stabilized}  if each component of $P_0$ intersects the boundary of $R_0$ in at least two intervals.
\end{definition}

This condition ensures that $(\widetilde{S}, \widetilde{P}, \tilde{h})$ is a partial open book whose pages embed into the pages of $(\{S_i\}_{i=0}^{2k}, h, \{\gamma_i\})$. As the term suggests, this condition may always be achieved by a sequence of positive stabilizations, and in fact, these may be chosen to occur on the $S_0$ page.  



\begin{theorem}\cite[Proposition 8.10]{LV} \label{thm:fobtopob}
With the notation above, the partial open book $(\widetilde{S},\widetilde{P},\widetilde{h})$ is compatible with a contact manifold $(\widetilde{M},\widetilde{\xi})$ which is
contactomorphic to $(M,\xi)$.  Furthermore, under this contactomorphism, the image of the dividing set of the characteristic foliation of $\xi$ on $\partial M$ divides $\mathcal{F}$. 
\end{theorem}



\begin{example} 
In this example, we return to the foliated open book of Example~\ref{ex:sorted}, which is not sufficiently stabilized.  Recall that $R'_0$ is constructed as a cornered neighborhood of the sorting arcs together with $A'_0$.  Observe that $P'_0:=S_0'\setminus R_0'$ consists of two bigons, each with an edge on $B$ and an edge on the annular $\partial R'_0$.  It follows that $S'_0$ cannot be built up from $R'_0$ by adding one-handles, which is the topological requirement for the surface\slash subsurface pair to define a partial open book.

\begin{figure}[h]
\begin{center}
\includegraphics[scale=1]{preliminaries/efobtorussuffstab3L}
\caption{ The shaded regions show the cornered neighborhoods $R_i''$ in each page of the sufficiently stabilized open book. As in Example~\ref{ex:sorted}, successive pages are identified by translation except  for the right-handed Dehn twist $\tau$  at $S_2''$.}\label{fig:sssorttorus}
\end{center}
\end{figure}

Figure~\ref{fig:sssorttorus} shows a sufficiently stabilized foliated open book for the same manifold, built by stabilizing along the dotted arc which  connected the two components of the binding.  The new monodromy is the composition of the original monodromy  with a positive Dehn twist along the circle formed by the core of the added handle and the stabilizing arc. 



 The new $P''_0:=S_0''\setminus R_0''$ is a single disk whose boundary intersects $\partial R''_0$ along two intervals; this ensures that $(\widetilde{S}'', \widetilde{P}'', \widetilde{h}'')$ is a partial open book.   In order to understand $\widetilde{h}''$, we first examine the flow of $P_0''$ through the manifold. Recall from Example~\ref{ex:sorted} that the only non-trivial identification between successive pages is a right-handed Dehn twist at the $S_2''$ page before the cut yielding $S_3''$.  The twist is along the core of the annular $R_2''$, so $P_4''$ is isotopic, relative to $A_4''=A_0''$, to $P_0''$.   Thus, the partial open book monodromy is simply the restriction of the foliated open book monodromy to $P_4''$.


\end{example}

As shown in \cite[Lemma 8.12]{LV}  the subsurfaces $R_i\subset S_i$ depend only on the foliation $\mathcal{F}$, rather than on the pages $S_i$. Construct the corresponding contact 3-manifold $(M,\xi,\mathcal{F})$ for a sorted abstract foliated open book $(\{S_i\},h,\{\gamma_i^\pm\})$. Recall from Definition~\ref{def:div} that the subsurface $R_+(\fol)$ (respectively $R_-(\fol)$) of $\partial M$ is a closed neighborhood of the (un)stable separatrices corresponding to positive (negative) hyperbolic points of $\mathcal{F}$. 

As noted in Section~\ref{sec:morse}, the graph of positive separatrices of $\nabla \pit$ from positive hyperbolic points on $\partial M$ is (non-smoothly)  isotopic to the graph of positive separatrices of $\fol$ from positive hyperbolic points on $\partial M$.  On the other hand, the former is isotopic through the stable critical submanifolds to a neighborhood of the sorting arcs $\cup_{H_+}\gamma^+_i$ on $S_0$.   This yields an identification between $R_+(\fol)\subset \partial M$ and $R_0\subset S_0$.  Similarly, studying negative separatrices of negative hyperbolic points  and unstable critical submanifolds yields an identification between $R_-(\fol)\subset \partial M$ and $R_{2k}\subset S_{2k}$. 

Similarly, all the $R_i$ can be identified with surfaces described only using the foliation $\fol$, independently of the foliated open book, as follows. Recall that $R_i$ is the (cornered) neighborhood of the union of $A_i$  and the intersection of all stable and unstable submanifolds of $\nabla \pi$ with $S_i$. Each of these intersections can be pushed up (or down) onto $\partial M$ along the corresponding stable (or unstable) submanifolds. While performing these isotopies we push the half-neighborhood of $A_i$ up along $I_+$ and down along $I_-$; the surface obtained after the isotopy is not a submanifold of $\partial M$, as it has a half twist in the middle of each component $I$ of $A_i$ which extends into the interior of $M$. See Figure \ref{fig:rtoq}.
\begin{figure}[h]
\begin{center}
\includegraphics[scale=.7]{preliminaries/RtoQ}
\caption{The blue region on the left-hand picture is the cornered neighborhood $R_i\subset S_i$.  On the right-hand figure, $R_i$ has been isotoped through $M$ in the direction of the indicated arrows to lie mostly on $\partial M$.  The small arrow indicates the half twist which extends into the interior of $M$. Note that $B$ has been blown up to $B\times I$ for clarity.}\label{fig:rtoq}
\end{center}
\end{figure}


    
\subsubsection{Gluing foliated open books.}\label{ssec:gluing} In order to glue foliated open books, we describe the matching conditions imposed upon their boundary foliations. 
Recall that a foliation $\fol$ on a surface $F$ always refers to the data of a signed foliation together with the function $\pit\colon F\setminus E\to S^1$ whose level sets are the leaves of $\fol$. 

\begin{definition} The \emph{reverse of a foliation $\fol$} on $F$ is the foliation on $-F$ which is equal to $\pit$ pointwise, but with the leaf orientations and signs of singular points reversed.  \end{definition}

The main advantage of foliated open books is that they are well suited for gluing. Suppose that  $(M^L,\xi^L,\mathcal{F}^L)$ and $(M^R,\xi^R,\fol^R)$ are foliated contact three-manifolds such that there exists  an orientation-reversing diffeomorphism $\psi\colon \partial M^L  \to \partial M^R$ that maps the reverse of the foliation $\fol^L$ onto $\fol^R$. 

Recall that by hypothesis, the boundary foliations  are  divided, so the boundaries $\partial M^{\bullet}$ are convex with respect to $\xi^{\bullet}$. (Here, and throughout this section, $\bullet$ will be an element of the set $\{R, L\}$.) Since the contact structures are $I$-invariant near the boundaries, $\psi$ determines a closed contact three-manifold \[(M,\xi)=(M^L\cup_\psi M^R,\xi^L\cup_\psi\xi^R).\]  

If the initial contact manifolds were supported by foliated open books $(\{S^L_i\},h^L)$ and  $(\{S^R_i\},h^R)$, respectively, then $(M,\xi)$ naturally inherits a supporting open book whose pages and binding are built by gluing the pages and bindings of the constituent pieces.  More precisely, recall that  $\partial S^{\bullet}_i=A_i^{\bullet}\cup B^{\bullet}$, where all the $B^{\bullet}$ are identified   when forming the manifolds $M^{\bullet}$.  The map $\psi$ identifies the intervals $A_i^L$ and $-A_i^R$ for all $i$, forming the surfaces \[S_i=S_i^L\bigcup_{A_i^L\xrightarrow{\psi}-A_i^R} S_i^R\] with boundary $B=B^L\cup B^R$.  Observe that a cut to $S_i^R$ pairs with a handle addition to $S_i^L$, and vice versa, so the surfaces  $S_i$  are  diffeomorphic  for all $i$.  This allows us to identify  $S_0\cong S_1 \cong\cdots \cong S_{2k}$ and we denote the composition of these identifications by  $\iota \colon S_0\to S_{2k}$.  Note that $\iota$  fixes $B$, {and it restricts to $P_{0}^\bullet$ as the identification $\iota^\bullet:P_0^\bullet \rightarrow P_{2k}^\bullet$  defined in Section \ref{sssec:suff}}. Letting $S:=S_0$,  the monodromy $h\colon S\to S$ for the glued-up open book can be obtained as the composition of $\iota $  with $h^L\cup h^R\colon S_{2k}=S_{2k}^L\cup S_{2k}^R\to S_{0}^L\cup S_{0}^R=S_0$. By construction, $h$ fixes $B$, as required.  


\begin{theorem}\cite[Theorem 6.2]{LV} \label{prop:glue} 
Suppose that the foliated open books $(\{S_i^L\},h^L)$ and $(\{S_i^R\},h^R)$ define the three-manifolds with foliated boundary
 $(M^L,\fol^L)$ and $(M^R,\fol^R)$, and assume that there is an orientation reversing diffeomorphism $\varphi\colon \partial M^L\to \partial M^R$ that takes the reverse of the foliation $\fol^L$ onto $\fol^R$. 

Then there are contact structures $\xi^L$ and $\xi^R$ supported by  $(\{S_i^L\},h^L)$ and $(\{S_i^R\},h^R)$, respectively, so that $\xi=\xi^L\cup_\varphi\xi^R$ is a contact structure $\xi$ on the manifold $M=M^L\cup_\varphi M^R$  that is supported by the honest open book $(S,h)$ constructed by pagewise gluing, as defined above.
\end{theorem}

Since $\iota \colon S_0\to S_{2k}$ is given as a sequence of identifications, the monodromy $h$ may be  difficult  to reconstruct in a complicated case, and the above construction does not automatically give a factorization in terms of  Dehn twists. For sorted open books, however, there is a straightforward way to describe $\iota$ (and thus $h$) as follows. 
Suppose now, that $(\{S^L_i\},h^L, \{\gamma_i^{\pm,L}\})$ and  $(\{S^R_i\},h^R,\{\gamma_i^{\mp,R}\})$ are sorted foliated open books compatible with 
 $(M^L,\xi^L,\mathcal{F}^L)$ and $(M^R,\xi^R,\fol^R)$, respectively. 
Recall that each page $S_i^{\bullet}$  decomposes as the union of a ``constant'' part $P_i^{\bullet}$ and an $i$-dependent part $R_i^{\bullet}$ which is determined by the foliation $\fol^{\bullet}$. By construction, $P_0^{\bullet}\cong P_1^{\bullet}\cong \cdots \cong P_{2k}^{\bullet}$. These diffeomorphisms are explicit in the construction of the pages $S_i^{\bullet}$ and together they determine $\iota\vert_{P_0^L\cup P_0^R}=\iota^L\cup \iota^R\colon P_0^L\cup P_0^R\to P_{2k}^L\cup P_{2k}^R$.


As  described earlier,  sorted foliated open books have the property that $R_0^L$ is isotopic in $M^L$ to $R_+(\fol^L)$.  This surface is mapped by $\psi$ onto $R_-(\fol^R)$, which in turn is isotopic in $M^R$ to $R_{2k}^R$. The composition of these three maps gives $\iota\vert_{R_0^L}\colon R_0^L\to R_{2k}^R$, and we can similarly obtain $\iota\vert_{R_0^R}\colon R_0^R\to R_{2k}^L$. This yields a concrete description of  the entire map $\iota$ on the remaining parts $R_{2k}^L\cup R_{2k}^L$. Together,  the above maps determine $h$ everywhere.  





 
 

